Computationally efficient joint coordination of multiple electric vehicle charging points using reinforcement learning

A major challenge in todays power grid is to manage the increasing load from electric vehicle (EV) charging. Demand response (DR) solutions aim to exploit flexibility therein, i.e., the ability to shift EV charging in time and thus avoid excessive peaks or achieve better balancing. Whereas the majority of existing research works either focus on control strategies for a single EV charger, or use a multi-step approach (e.g., a first high level aggregate control decision step, followed by individual EV control decisions), we rather propose a single-step solution that jointly coordinates multiple charging points at once. In this paper, we further refine an initial proposal using reinforcement learning (RL), specifically addressing computational challenges that would limit its deployment in practice. More precisely, we design a new Markov decision process (MDP) formulation of the EV charging coordination process, exhibiting only linear space and time complexity (as opposed to the earlier quadratic space complexity). We thus improve upon earlier state-of-the-art, demonstrating 30% reduction of training time in our case study using real-world EV charging session data. Yet, we do not sacrifice the resulting performance in meeting the DR objectives: our new RL solutions still improve the performance of charging demand coordination by 40-50% compared to a business-as-usual policy (that charges EV fully upon arrival) and 20-30% compared to a heuristic policy (that uniformly spreads individual EV charging over time).

==> authors/Authors_info.tex <==

\cleardoublepage
\bio{authors/Manuphoto}
Manu Lahariya is a doctoral student in the Internet Technology and Data Science Lab (IDLab) at Ghent University - imec, Ghent, Belgium. His doctoral research focuses on the development of machine learning algorithms for modeling Electric Vehicle (EV) session data and the application of deep reinforcement learning such as Q-networks for Model Predictive Control (MPC) of Electric vehicle (EV) charging stations. He also has experience in development of time series algorithms for sales forecasting. He obtained his Masters’ and Bachelors’ degree in Aerospace Engineering from Indian Institute of Technology (IIT) Kharagpur (2012-2017). 
\endbio

\vspace{20}

\bio{authors/Nasrinphoto}
Nasrin Sadeghianpourhamami is an AI scientist/researcher at BluWave-Ai with a proven record of successfully applying AI in 4 major industry projects. She received her doctorate in computer science engineering in from Ghent University - imec, Ghent, Belgium (2018). She has worked on statistical modelling of real-world data, developing data-driven control via deep reinforcement learning, and has contributed in facilitating the integration of sustainable energy production/consumption in the evolving power grid.
\endbio

\vspace{20}

\bio{authors/ChrisPhoto}
Chris Develder is associate professor with the research group IDLab in the Dept. of Information Technology (INTEC) at Ghent University - imec, Ghent, Belgium. He currently leads two research teams within IDLab, one on converting text to knowledge (i.e., NLP, mostly information extraction using machine learning), the other on data analytics and machine learning for smart grids. He regularly serves as reviewer/TPC member for international journals and conferences (IEEE/ACM Trans. Networking, IEEE Trans. Smart Grid, Energy and Buildings; EMNLP, ACL, ACM SIGIR, ACM CIKM, IEEE SmartGridComm, etc.). He is Senior Member of IEEE, Member of ACM, and Member of ACL. 
\endbio
